Towards Efficient Exact Optimization of Language Model Alignment

The alignment of language models with human preferences is vital for their application in real-world tasks. The problem is formulated as optimizing the model's policy to maximize the expected reward that reflects human preferences with minimal deviation from the initial policy. While considered as a straightforward solution, reinforcement learning (RL) suffers from high variance in policy updates, which impedes efficient policy improvement. Recently, direct preference optimization (DPO) was proposed to directly optimize the policy from preference data. However, we show that DPO derived based on the optimal solution of the problem leads to a compromised mean-seeking approximation of the optimal solution in practice. In this paper, we propose efficient exact optimization (EXO) of the alignment objective. EXO is guaranteed to optimize in the same direction as RL algorithms asymptotically for arbitrary policy parametrization. This leads to the same mode-seeking solution, while enables efficient optimization by circumventing the complexities of RL. We also compare our method to DPO with both theoretical and empirical analyses, and further demonstrate the advantages of our method over existing approaches on realistic human preference data. Code is available at https://github.com/haozheji/exact-optimization.

==> method_misc.tex <==
% product of experts ===============================

We first start with the setting of Eq \eqref{equ:lhf_objective} which assumes the existence of the SFT policy $\pisft$ and the reward model $r$. Given an input prompt $\x$, \hnote{if we defined it, it should be estimated. Since we want to differentiate ourselves from DPO, maybe we should directly ``define Eq. \eqref{eq:r_theta}''.} we first define the estimated reward function on the prefix $\y_{\le t}$ of the complete generation $\y$ modeled by the policy $\pi_\theta$:
\begin{equation}
    \label{equ:reward_prefix}
    r_\theta(\x, \y_{\le t}) = \gamma \log \frac{\pi_\theta(\y_{\le t}|\x)}{\pisft(\y_{\le t}|\x)},
\end{equation}
where $\gamma>0$ is a scaling factor. We define $\pi_{\theta, \gamma}(\y_{\le t}|\x)\propto \pi_{\theta}(\y_{\le t}|\x)^\gamma \pisft(\y_{\le t}|\x)^{1-\gamma}$ as the Product of Experts~\citep{PoE} between the distribution of $\pi_\theta$ and $\pisft$ with the exponent $\gamma$ and $1-\gamma$ respectively. Specifically, for $\gamma=1$, $\pi_{\theta,\gamma}=\pi_\theta$. Then we rearrange Eq \eqref{equ:reward_prefix} using $\pi_{\theta,\gamma}$:
\begin{equation}
\label{eq:r_theta}
    r_\theta(\x, \y_{\le t})=\log \frac{
        \pi_{\theta, \gamma}(\y_{\le t}|\x)
        }{\pisft(\y_{\le t}|\x)} + \log Z_{\theta, \gamma}(\x),
\end{equation}
where $Z_{\theta,\gamma}(\x)=\sum_{\y_{\le t}} \pi_{\theta}(\y_{\le t}|\x)^\gamma \pisft(\y_{\le t}|\x)^{1-\gamma}$ is the partition function that only depends on $\x$.


% general form and final time steps ===============



\begin{align}
    \label{equ:general_exact}
    \Lexact(\pi_{\theta,\gamma}) &=
    \mathbb{E}_{\pisft(\ysamp{1:N}|\x)}
    \mathbb{E}_{p(\tsamp{1:N}|\ysamp{1:N})}
    \Big[\nonumber\\
    &\KLDiv\big(
    p_{r_\theta}(i|\ysamp{1:N}_{\le\tsamp{1:N}}, \x)\|
    p_{r}(i|\ysamp{1:N}, \x)\big
    )
    \Big],
\end{align}
where $p(\tsamp{1:N}|\ysamp{1:N})=\prod_{i=1}^N p(\tsamp{i}|\ysamp{i})$. Next, we consider two special cases of this general objective with different instantiation of $p(t|y)$ and illustrate the correspondance with the alignment objective of Eq \eqref{equ:lhf_objective}. 


\paragraph{Supervision on Final Time Steps Only.} The first form only uses the final time step of each sampled sequence to calculate the loss by setting $p(t|\y)=\1[t - T(\y)]$ where $T(\y)$ is the length of the sequence $\y$. With this setup, $\ysamp{1:N}_{\le \tsamp{1:N}}=\ysamp{1:N}$, so $p_{r_\theta}$ is now defined on the complete sequence of the $N$ samples $\ysamp{1:N}$. We rewrite Eq \eqref{equ:general_exact} into the following form which has supervision only on the final time steps:
\begin{align}
    &\Lexactfinal(\pi_{\theta,\gamma})=
    \mathbb{E}_{\pisft(\ysamp{1:N}|\x)}
    \Big[\nonumber\\
    &\quad \quad \quad \quad \KLDiv\big(
    p_{r_\theta}(i|\ysamp{1:N}, \x)\|
    p_{r}(i|\ysamp{1:N},\x)\big
    )
    \Big].
\end{align}


% random time steps ===============================




\paragraph{Supervision on Random Time Steps Uniformly.}The second form draws time steps uniformly from all steps of the sampled sequence independently, i.e., $\tsamp{i}\sim \U{\{1,T(\ysamp{i})\}}$. We rewrite Eq \eqref{equ:general_exact} into the following form that supervises random intermediate time steps of the sequence:
\begin{align}
    \label{equ:exact_uniform}
    &\Lexactuniform(\pi_{\theta,\gamma}) =
    \mathbb{E}_{\pisft(\ysamp{1:N}|\x)}
    \mathbb{E}_{\tsamp{1:N}\sim\U\{1,T(\ysamp{1:N})\}}
    \Big[\nonumber\\
    &\quad \quad \quad \ \ \KLDiv\big(
    p_{r_\theta}(i|\ysamp{1:N}_{\le\tsamp{1:N}}, \x)\|
    p_{r}(i|\ysamp{1:N}, \x)\big
    )
    \Big].
\end{align}

Intuitively, the probability of the policy $\pi_\theta(\ysamp{i}_{\le \tsamp{i}}|\x)$ on each prefix of the sample $\ysamp{i}_{\le \tsamp{i}}$ is provided with direct supervision from the reward of the complete sequence sample $r(\x,\ysamp{i})$. Compared to $\Lexactfinal$ that only has supervision on the final time steps, the supervising signals on the intermediate time steps of the sequence is crucial for stable training of the auto-regressive policy. Next, we show that this intermediate supervision is indeed meaningful by connecting it with the alignment objective on the prefix as defined in Definition \ref{def:prefix_alignment}.

\begin{restatable}{definition}{PrefixAlignmentDef}
\label{def:prefix_alignment}
    Given $1\le t \le T$ 
    %where $T_{\max}=\max_{\y\sim \pi_\theta(\y|\x)} T(\y)$
    , the alignment objective $\Jlhf^t(\pi_{\theta,\gamma})$ on the prefix with length $t$ is defined as:
    \begin{align}
        \Jlhf^t(\pi_{\theta,\gamma}) &= \mathbb{E}_{\pi_{\theta,\gamma}(\y_{\le t}|\x)}\Big[ 
        \Rinterm_t(\x, \y_{\le t})
        \Big] \nonumber\\
        &- \beta \KLDiv[\pi_{\theta,\gamma}(\y_{\le t}|\x)\|\pisft(\y_{\le t}|\x)],
    \end{align}
where $\Rinterm_t(\x, \y_{\le t}) = \log\mathbb{E}_{
    \pisft(\y_{> t}|\y_{\le t})
}
[
    e^{\frac{1}{\beta}r(\x, \y_{\le t}, \y_{> t})}
]$ is defined as the \textit{intermediate reward} of the prefix $y_{\le t}$.% with length $t$.
\end{restatable}

This definition is motivated by the form of the optimal policy $\pi_{\theta^*,\gamma}$ on the prefix $\y_{\le t}$:
\begin{equation}
    \label{equ:optimal_prefix}
    \pi_{\theta^*,\gamma}(\y_{\le t}|\x) = \pisft(\y_{\le t}|\x)\frac{
        e^{\Rinterm_t(\x, \y_{\le t})}
    }{Z(\x)}.
\end{equation}
In this form, the optimal policy on the prefix $\y_{\le t}$ is proportional to the product of the SFT policy on $\y_{\le t}$ and the exponential \textit{intermediate reward} $e^{\Rinterm_t(\x, \y_{\le t})}$, which is the expectation of the exponential reward by marginalizing out the future continuation $\y_{> t}$ sampled from the SFT policy given the prefix $\y_{\le t}$. In reminisence of the alignment objective on the complete sequence, $\Jlhf^t(\pi_{\theta,\gamma})$ is defined in the KL-regularized reward maximization formulation whose optimal solution is the same solution of $\Jlhf(\pi_{\theta,\gamma})$ defined on prefix $\y_{\le t}$. Finally, we summarize the relationship of $\Lexactuniform(\pi_{\theta,\gamma})$ and $\Jlhf^t(\pi_{\theta,\gamma})$ in Theorem \ref{theorem:rel_lhf_prefix}.
\begin{restatable}{theorem}{ExactIntermTheorem}
\label{theorem:rel_lhf_prefix}
$\Lexactuniform(\pi_{\theta,\gamma})
\ge
-\beta \mathbb{E}_{t\sim \U\{1,T\}}
[
\Jlhf^t(\pi_{\theta,\gamma})
]$ given arbitary $\theta$, for $N\rightarrow\infty$.
\end{restatable}
According to Theorem \ref{theorem:rel_lhf_prefix}, we are justified that minimizing $\Lexactuniform(\pi_{\theta,\gamma})$ is equivalent to maximizing the lower bound of $\Jlhf^t(\pi_{\theta,\gamma})$ with $t$ uniformly sampled from all possible time steps, which encourages the convergence to the optimal policy at all prefix length. We provide an intuitive understanding of supervising the policy on the prefix with the rewarding signal of the complete generation, i,e, the policy is guided with expected return in the future based on the given prefix.

